Joint Channel Estimation, Activity Detection and Decoding using Dynamic Message-Scheduling for Machine-Type Communications

In this work, we present a joint channel estimation, activity detection and data decoding scheme for massive machine-type communications. By including the channel and the a priori activity factor in the factor graph, we present the bilinear message-scheduling GAMP (BiMSGAMP), a message-passing solution that uses the channel decoder beliefs to refine the activity detection and data decoding. We include two message-scheduling strategies based on the residual belief propagation and the activity user detection in which messages are evaluated and scheduled in every new iteration. An analysis of the convergence of BiMSGAMP along with a study of its computational complexity is carried out. Numerical results show that BiMSGAMP outperforms state-of-the-art algorithms, highlighting the gains achieved by using the dynamic scheduling strategies and the effects of the channel decoding part in the system.

==> BiMSGAMP_SE_alg.tex <==
% State-evolution pseudocode
% -------------------------------------------------------------------------
\newcounter{CounterSE}
    \begin{table}[H]
        %\footnotesize
        %\scriptsize
            \label{tab:SE}
            \begin{tabular}{ll}\hline
                \multicolumn{2}{l}{\textbf{Algorithm 2} {State Evolution of BiMSGAMP}}           \\ \hline
                % --------------------------------------------------------------------------
                % ----------------------------------------------------------------------------
                \multicolumn{2}{l}{\textbf{output} $\textsf{mse}_x^{I} = \chi_x^{I} - \varrho_x^{I}$ and $\textsf{mse}_h^{I} = \chi_h^{I} - \varrho_h^{I}$}\\
                % Start repeat ---------------------------------------------------------------
                \multicolumn{2}{l}{\textbf{for} $i=1,\dots,I$}                \\
                % New line -----------------------
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\chi_x^{i} = \int (x^{i})^2\, \sum_c \sum_s \mathcal{P}\!\left(x,c,s\right)\text{d}x$ \\[4pt] 
                % New line -----------------------
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\chi_h^{i} = \int (h^{i})^2\, \mathcal{P}\!\left(h;\hat{\rho}\right)\text{d}h$ \\[4pt]
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\chi_z^{i} = |\mathcal{S}^{i}| \chi_x^{i} \chi_h^{i}$ \\[4pt]  
                % New line -----------------------
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\varrho_z^{i} = \int \frac{\left[\int z\,p_{y|z}\left(y|z\right)\mathcal{N}_c\left(z|\sqrt{|\mathcal{S}^{i}|\varrho_x\varrho_h}\,\iota,\nu^p\right)\text{d}z\right]^2}{\int p_{y|z}\left(y|z\right)\mathcal{N}_c\left(z|\sqrt{|\mathcal{S}^{i}|\varrho_x\varrho_h}\,\iota,\nu^p\right)\text{d}z}\text{D}\iota\,\text{d}y$ \\[4pt]                 
                % New line -----------------------
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\nu^{ri} = \frac{|\mathcal{S}^{i}|^2\left(\chi_x \chi_h - \varrho_x \varrho_h\right)^2}{M \varrho_h\left(\varrho_z - |\mathcal{S}^{i}| \varrho_x \varrho_h\right)}$ \\[4pt]  
                % New line -----------------------
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\nu^{qi} = \frac{|\mathcal{S}^{i}|^2\left(\chi_x \chi_h - \varrho_x \varrho_h\right)^2}{T \varrho_x\left(\varrho_z - |\mathcal{S}^{i}| \varrho_x \varrho_h\right)}$ \\[4pt]                  
                % New line -----------------------
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\varrho_x^{i} = \int \frac{\left[\int x\, \sum_c \sum_s \mathcal{P}\!\left(x,c,s\right)\mathcal{N}_c\left(x|\zeta,\nu^r\right)\text{d}x\right]^2}{\int \sum_c \sum_s \mathcal{P}\!\left(x,c,s\right)\mathcal{N}_c\left(x|\zeta,\nu^r\right)\text{d}x}\, \text{d}\zeta$ \\[4pt]                 
                % New line -----------------------
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\varrho_h^{i} = \int \frac{\left[\int h\, \mathcal{P}\!\left(h;\hat{\rho}\right)\mathcal{N}_c\left(h|\zeta,\nu^r\right)\text{d}h\right]^2}{\int \mathcal{P}\!\left(h|\hat{\rho}\right)\mathcal{N}_c\left(h|\zeta,\nu^r\right)\text{d}h}\, \text{d}\zeta$ \\[4pt]    
                % New line -----------------------
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\nu^{pi} =\, |\mathcal{S}^{i}|\left(\chi_x^{i} \chi_h^{i} - \varrho_x^{i} \varrho_h^{i}\right)$ \\[4pt]
                % New line -----------------------
                \stepcounter{CounterSE} 
                %
                {{\scriptsize [\theCounterSE]}}  &  $\hat{\rho}^{i} = \frac{\mathcal{N}_c\left(0 | \hat{r}, \nu^r + \chi_x\right)}{\mathcal{N}_c\left(0 | \hat{r}, \nu^r + \chi_x\right) + \mathcal{N}_c\left(0 | \hat{r}, \nu^r\right)}$ \\[4pt]
                % ----------------------------------------------------------------------------
                % End repeat ---------------------------------------------------------------
                \multicolumn{2}{l}{\textbf{end}} \\ \hline
            \end{tabular}
    \end{table}


	    
	   
        

==> RBP.tex <==
% Algorithm pseudocode
% -------------------------------------------------------------------------
\newcounter{RBPCounterDef}
\newcounter{RBPCounter}
    \begin{table}[t]
        %\footnotesize
            \begin{tabular}{p{0.2cm}p{0.2cm}ll}
                \hline
                \multicolumn{4}{l}{\footnotesize\textbf{Algorithm 2} {Residual Belief Propagation based Message Scheduling}}           \\ \hline
                % ----------------------------------------------------------------------------
                % Start definition -----------------------------------------------------------
                \multicolumn{4}{l}{\textbf{initialize}}            \\
                % New line
                \stepcounter{RBPCounter} 
                {[{\scriptsize A\theRBPCounter}]}  & \multicolumn{3}{l}{$l=1$, $N$, $\mathcal{S}^{(i)}$, $\hat{\bh}^{(i)}$, $\hat{\mathbf{r}}^{(i)}$, $\Delta^{r(i)}$, $\Delta^{h(i)}$}\\
                % ----------------------------------------------------------------------------
                % Start if ---------------------------------------------------------------
                & \multicolumn{3}{l}{\textbf{if} $\left(|\mathcal{S}^{(i)}| = 0\right)$}\\
                % New line
                & & \multicolumn{2}{l}{$\forall n$, \textbf{if} $\left(\text{Res}\left(\nu_{nm}\left(h_{nm}\right)\right) > \textit{the first other }|\hat{\boldsymbol{\rho}}^{(i)}| \textit{residuals}\right)$}\\            
                % New line
                \stepcounter{RBPCounter} 
                {[{\scriptsize A\theRBPCounter}]} & & \multicolumn{2}{l}{$\mathcal{S}^{(i+1)}_l = n$ and $l = l+1$}\\             
                % New line
                & & \multicolumn{2}{l}{\textbf{end if}}\\                
                & \multicolumn{3}{l}{\textbf{else}} \\                            
                % New line
                \stepcounter{RBPCounter} 
                {[{\scriptsize A\theRBPCounter}]}  & &\multicolumn{2}{l}{ Remove the first element of $\mathcal{S}^{(i)}$, that is, $\mathcal{S}^{(i+1)} = \left[\mathcal{S}^{(i)}_2, \dots, \mathcal{S}^{(i)}_{|\mathcal{S}^{(i)}|}\right]$}\\ 
                % New line
                & \multicolumn{3}{l}{\textbf{end if}} \\         
                % New line
                \stepcounter{RBPCounter} 
                {[{\scriptsize A\theRBPCounter}]}  & \multicolumn{3}{l}{$\forall \left(n \notin \mathcal{S}^{(i+1)}\right)$ and $m$,}\\ 
                % New line
                \stepcounter{RBPCounter} 
                {[{\scriptsize A\theRBPCounter}]}  & & \multicolumn{2}{l}{$\hat{h}_{nm}^{(i+1)} = \hat{h}_{nm}^{(i)}$;\hspace{0.5cm} $\nu^{h(i+1)}_{nm} = \nu^{h(i)}_{nm}$; \hspace{0.5cm}$\hat{r}_{nm}^{(i+1)} = \hat{r}_{nm}^{(i)}$;\hspace{0.5cm} $\nu^{r(i+1)}_{nm} = \nu^{r(i)}_{nm}$}\\ \hline
            \end{tabular}
    \end{table}


	    

